TabPFN: A Transformer That Solves Small Tabular Classification Problems in a Second

We present TabPFN, a trained Transformer that can do supervised classification for small tabular datasets in less than a second, needs no hyperparameter tuning and is competitive with state-of-the-art classification methods. TabPFN performs in-context learning (ICL), it learns to make predictions using sequences of labeled examples (x, f(x)) given in the input, without requiring further parameter updates. TabPFN is fully entailed in the weights of our network, which accepts training and test samples as a set-valued input and yields predictions for the entire test set in a single forward pass. TabPFN is a Prior-Data Fitted Network (PFN) and is trained offline once, to approximate Bayesian inference on synthetic datasets drawn from our prior. This prior incorporates ideas from causal reasoning: It entails a large space of structural causal models with a preference for simple structures. On the 18 datasets in the OpenML-CC18 suite that contain up to 1 000 training data points, up to 100 purely numerical features without missing values, and up to 10 classes, we show that our method clearly outperforms boosted trees and performs on par with complex state-of-the-art AutoML systems with up to 230$\times$ speedup. This increases to a 5 700$\times$ speedup when using a GPU. We also validate these results on an additional 67 small numerical datasets from OpenML. We provide all our code, the trained TabPFN, an interactive browser demo and a Colab notebook at https://github.com/automl/TabPFN.

==> figures/ablations/abl_train_scaling.tex <==
\begin{tabular}{lll}
\toprule
{} & Tabular PFN (Train Statistics Only) & Tabular PFN (Train + Test Statistics) \\
\midrule
Wins AUC OVO      &                           4 &                         \textbf{9} \\
Wins Acc.         &                 \textbf{12} &                                  7 \\
Wins CE           &                           6 &                        \textbf{17} \\
Win/T/L AUC &                        &                             9/17/4 \\
Win/T/L Acc &                       &                            7/11/12 \\
Win/T/L CE  &                       &                             17/7/6 \\
Mean AUC OVO      &           0.8941$\pm$0.01 &           \textbf{0.8944}$\pm$0.01 \\
Mean Acc.         &    \textbf{0.8265}$\pm$0.01 &                   0.8262$\pm$0.011 \\
Mean CE           &             0.731$\pm$0.015 &          \textbf{0.7302}$\pm$0.015 \\
\bottomrule
\end{tabular}


==> figures/ablations/diff_ablation.tex <==
\begin{tabular}{lll}
\toprule
Ablation & Differentiable hyperparameter tuning & No differentiable hyperparameter tuning \\
\midrule
Mean CE      &                      0.733$\pm$0.014 &                        0.735$\pm$0.013 \\
Mean ROC AUC &                     0.8942$\pm$0.002 &                         0.8939$\pm$0.003 \\
\bottomrule
\end{tabular}


==> figures/ablations/ensembling_matrix.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\end{tikzpicture}


==> figures/ablations/rotate_feats_2.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.194607843137255,0.453431372549019,0.632843137254902}
\definecolor{color1}{rgb}{0.881862745098039,0.505392156862745,0.173039215686275}

\begin{axis}[
height=5cm,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=5cm,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=3.5,
xtick style={color=black},
xtick={0,1,2,3},
xticklabel style={rotate=45.0},
xticklabels={Catboost,Log. Regr.,MLP,TabPFN},
y grid style={white!69.0196078431373!black},
ylabel={ROC AUC},
ymin=0.859432973181843, ymax=0.901096664837093,
ytick style={color=black},
ytick={0.855,0.86,0.865,0.87,0.875,0.88,0.885,0.89,0.895,0.9,0.905}
]
\path [draw=white!24.7058823529412!black, fill=color0, line width=1.5pt]
(axis cs:-0.396,0.884586307078087)
--(axis cs:-0.004,0.884586307078087)
--(axis cs:-0.004,0.889356889711043)
--(axis cs:-0.396,0.889356889711043)
--(axis cs:-0.396,0.884586307078087)
--cycle;
\path [draw=white!24.7058823529412!black, fill=color1, line width=1.5pt]
(axis cs:0.004,0.867384981687053)
--(axis cs:0.396,0.867384981687053)
--(axis cs:0.396,0.872844751602193)
--(axis cs:0.004,0.872844751602193)
--(axis cs:0.004,0.867384981687053)
--cycle;
\path [draw=white!24.7058823529412!black, fill=color0, line width=1.5pt]
(axis cs:0.604,0.862144120831149)
--(axis cs:0.996,0.862144120831149)
--(axis cs:0.996,0.865054445339392)
--(axis cs:0.604,0.865054445339392)
--(axis cs:0.604,0.862144120831149)
--cycle;
\path [draw=white!24.7058823529412!black, fill=color1, line width=1.5pt]
(axis cs:1.004,0.862158330224286)
--(axis cs:1.396,0.862158330224286)
--(axis cs:1.396,0.865039146564893)
--(axis cs:1.004,0.865039146564893)
--(axis cs:1.004,0.862158330224286)
--cycle;
\path [draw=white!24.7058823529412!black, fill=color0, line width=1.5pt]
(axis cs:1.604,0.875803757530548)
--(axis cs:1.996,0.875803757530548)
--(axis cs:1.996,0.879171779874893)
--(axis cs:1.604,0.879171779874893)
--(axis cs:1.604,0.875803757530548)
--cycle;
\path [draw=white!24.7058823529412!black, fill=color1, line width=1.5pt]
(axis cs:2.004,0.876855167039785)
--(axis cs:2.396,0.876855167039785)
--(axis cs:2.396,0.878355748526997)
--(axis cs:2.004,0.878355748526997)
--(axis cs:2.004,0.876855167039785)
--cycle;
\path [draw=white!24.7058823529412!black, fill=color0, line width=1.5pt]
(axis cs:2.604,0.891385240402914)
--(axis cs:2.996,0.891385240402914)
--(axis cs:2.996,0.897295084295591)
--(axis cs:2.604,0.897295084295591)
--(axis cs:2.604,0.891385240402914)
--cycle;
\path [draw=white!24.7058823529412!black, fill=color1, line width=1.5pt]
(axis cs:3.004,0.890088755571084)
--(axis cs:3.396,0.890088755571084)
--(axis cs:3.396,0.89555942974199)
--(axis cs:3.004,0.89555942974199)
--(axis cs:3.004,0.890088755571084)
--cycle;
\draw[draw=white!24.7058823529412!black,fill=color0,line width=0.75pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=white!24.7058823529412!black,fill=color0,line width=0.75pt}
\addlegendentry{False}

\draw[draw=white!24.7058823529412!black,fill=color1,line width=0.75pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=white!24.7058823529412!black,fill=color1,line width=0.75pt}
\addlegendentry{True}

\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
-0.2 0.884586307078087
-0.2 0.883660774312101
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
-0.2 0.889356889711043
-0.2 0.889727392766034
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
-0.298 0.883660774312101
-0.102 0.883660774312101
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
-0.298 0.889727392766034
-0.102 0.889727392766034
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.2 0.867384981687053
0.2 0.864422580960724
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.2 0.872844751602193
0.2 0.872952464877505
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.102 0.864422580960724
0.298 0.864422580960724
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.102 0.872952464877505
0.298 0.872952464877505
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.8 0.862144120831149
0.8 0.86132677734799
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.8 0.865054445339392
0.8 0.866492382333444
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.702 0.86132677734799
0.898 0.86132677734799
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.702 0.866492382333444
0.898 0.866492382333444
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.2 0.862158330224286
1.2 0.861365373056933
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.2 0.865039146564893
1.2 0.866495317946046
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.102 0.861365373056933
1.298 0.861365373056933
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.102 0.866495317946046
1.298 0.866495317946046
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.8 0.875803757530548
1.8 0.873318633039343
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.8 0.879171779874893
1.8 0.879324688228127
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.702 0.873318633039343
1.898 0.873318633039343
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.702 0.879324688228127
1.898 0.879324688228127
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.2 0.876855167039785
2.2 0.874610773362992
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.2 0.878355748526997
2.2 0.878355748526997
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.102 0.874610773362992
2.298 0.874610773362992
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.102 0.878355748526997
2.298 0.878355748526997
};
\addplot [line width=1pt, black, mark=diamond*, mark size=2.5, mark options={solid,fill=white!24.7058823529412!black}, only marks, forget plot]
table {%
2.2 0.88061614959087
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.8 0.891385240402914
2.8 0.890724362138769
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.8 0.897295084295591
2.8 0.899202860670945
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.702 0.890724362138769
2.898 0.890724362138769
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.702 0.899202860670945
2.898 0.899202860670945
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
3.2 0.890088755571084
3.2 0.889833787274339
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
3.2 0.89555942974199
3.2 0.896046167610741
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
3.102 0.889833787274339
3.298 0.889833787274339
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
3.102 0.896046167610741
3.298 0.896046167610741
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
-0.396 0.889111149178273
-0.004 0.889111149178273
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.004 0.870422028656478
0.396 0.870422028656478
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
0.604 0.864276097660003
0.996 0.864276097660003
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.004 0.864254125242626
1.396 0.864254125242626
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
1.604 0.877633754420465
1.996 0.877633754420465
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.004 0.877845051953799
2.396 0.877845051953799
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
2.604 0.89605609749986
2.996 0.89605609749986
};
\addplot [line width=1.5pt, white!24.7058823529412!black, forget plot]
table {%
3.004 0.893258326853564
3.396 0.893258326853564
};
\end{axis}

\end{tikzpicture}


==> figures/diffable_prior/diff_inferred_params_lengthscale.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Length Scale},
xmin=-0.520911949125796, xmax=10.4343094087474,
xtick style={color=black},
xtick={-2,0,2,4,6,8,10,12},
y grid style={white!69.0196078431373!black},
%ylabel={Cross entropy Loss},
ymin=0.597367018461227, ymax=0.619568020105362,
ytick style={color=black},
ytick={0.6,0.61,0.62},
mystylepalette,
mystylepalettehptuning,
]
\addplot [line width=1.5pt, color0]
table {%
-0.0229473419497435 0.618558883666992
0.121390225347663 0.612334966659546
0.26572779264507 0.607292473316193
0.410065359942476 0.603575825691223
0.554402927239883 0.601081132888794
0.698740494537289 0.599564909934998
0.843078061834696 0.598755121231079
0.987415629132102 0.598417460918427
1.13175319642951 0.598376154899597
1.27609076372692 0.598509907722473
1.42042833102432 0.598738789558411
1.56476589832173 0.599012494087219
1.70910346561914 0.599299728870392
1.85344103291654 0.599582195281982
1.99777860021395 0.59984940290451
2.14211616751135 0.600096106529236
2.28645373480876 0.600320219993591
2.43079130210617 0.600521981716156
2.57512886940357 0.600702524185181
2.71946643670098 0.600863754749298
2.86380400399839 0.601008057594299
3.00814157129579 0.601137578487396
3.1524791385932 0.601254820823669
3.29681670589061 0.601361870765686
3.44115427318801 0.601460516452789
3.58549184048542 0.601552426815033
3.72982940778283 0.601639151573181
3.87416697508023 0.601721823215485
4.01850454237764 0.60180139541626
4.16284210967505 0.601878643035889
4.30717967697245 0.601954162120819
4.45151724426986 0.602028489112854
4.59585481156727 0.602101981639862
4.74019237886467 0.602174937725067
4.88452994616208 0.602247476577759
5.02886751345949 0.602319836616516
5.17320508075689 0.602391958236694
5.3175426480543 0.602464079856873
5.46188021535171 0.602536022663116
5.60621778264911 0.602607786655426
5.75055534994652 0.602679431438446
5.89489291724392 0.602750718593597
6.03923048454133 0.602821707725525
6.18356805183874 0.602892339229584
6.32790561913614 0.602962255477905
6.47224318643355 0.603031516075134
6.61658075373096 0.603100061416626
6.76091832102836 0.603167772293091
6.90525588832577 0.603234350681305
7.04959345562318 0.603299915790558
7.19393102292058 0.603364169597626
7.33826859021799 0.603427112102509
7.4826061575154 0.603488624095917
7.6269437248128 0.60354870557785
7.77128129211021 0.603607177734375
7.91561885940762 0.603664040565491
8.05995642670502 0.603719294071198
8.20429399400243 0.603772759437561
8.34863156129984 0.603824555873871
8.49296912859724 0.603874683380127
8.63730669589465 0.603923082351685
8.78164426319206 0.603969752788544
8.92598183048946 0.604014754295349
9.07031939778687 0.604058027267456
9.21465696508428 0.604099750518799
9.35899453238168 0.604140043258667
9.50333209967909 0.604178607463837
9.6476696669765 0.604215741157532
9.7920072342739 0.604251563549042
9.93634480157131 0.604285955429077
};
\addplot [line width=1.5pt, red]
table {%
1.06460619112069 0.597367018461227
1.06460619112069 0.619568020105362
};
\addplot [line width=1.5pt, color0, dashed]
table {%
1 0.597367018461227
1 0.619568020105362
};
\end{axis}

\end{tikzpicture}


==> figures/diffable_prior/diff_inferred_params_noise.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Noise},
xmin=-0.0260454922471704, xmax=0.521715466094274,
xtick style={color=black},
xtick={-0.1,0,0.1,0.2,0.3,0.4,0.5,0.6},
y grid style={white!69.0196078431373!black},
%ylabel={Cross entropy Loss},
ymin=0.59209563434124, ymax=0.598774948716164,
ytick style={color=black},
ytick={0.593,0.598},
mystylepalette,
mystylepalettehptuning,
]
\addplot [line width=1.5pt, color0]
table {%
-0.00114726686801381 0.597987830638885
0.00606961005348086 0.597328543663025
0.0132864869749755 0.596720576286316
0.0205033638964702 0.596159875392914
0.0277202408179648 0.595644533634186
0.0349371177394595 0.595174372196198
0.0421539946609541 0.594749987125397
0.0493708715824488 0.594371557235718
0.0565877485039434 0.594038367271423
0.0638046254254381 0.593748927116394
0.0710215023469327 0.593500435352325
0.0782383792684274 0.5932896733284
0.0854552561899221 0.593112766742706
0.0926721331114167 0.592965483665466
0.0998890100329114 0.592844069004059
0.107105886954406 0.592744648456573
0.114322763875901 0.592663943767548
0.121539640797395 0.592598736286163
0.12875651771889 0.59254652261734
0.135973394640385 0.592505156993866
0.143190271561879 0.592472612857819
0.150407148483374 0.592447519302368
0.157624025404869 0.592428684234619
0.164840902326363 0.59241509437561
0.172057779247858 0.59240597486496
0.179274656169353 0.592400789260864
0.186491533090847 0.5923992395401
0.193708410012342 0.592400789260864
0.200925286933837 0.592405498027802
0.208142163855331 0.592413127422333
0.215359040776826 0.592423796653748
0.222575917698321 0.592437565326691
0.229792794619815 0.592454493045807
0.23700967154131 0.592474699020386
0.244226548462804 0.592498481273651
0.251443425384299 0.592525899410248
0.258660302305794 0.592557549476624
0.265877179227288 0.592593431472778
0.273094056148783 0.592634081840515
0.280310933070278 0.592679738998413
0.287527809991772 0.592730760574341
0.294744686913267 0.592787623405457
0.301961563834762 0.592850625514984
0.309178440756256 0.592920362949371
0.316395317677751 0.592997193336487
0.323612194599246 0.593081593513489
0.33082907152074 0.593173921108246
0.338045948442235 0.593274831771851
0.34526282536373 0.593384683132172
0.352479702285224 0.593503892421722
0.359696579206719 0.593633055686951
0.366913456128214 0.593772649765015
0.374130333049708 0.593922972679138
0.381347209971203 0.594084620475769
0.388564086892698 0.594258010387421
0.395780963814192 0.594443500041962
0.402997840735687 0.594641625881195
0.410214717657182 0.59485250711441
0.417431594578676 0.595076620578766
0.424648471500171 0.595314264297485
0.431865348421665 0.595565736293793
0.43908222534316 0.595831155776978
0.446299102264655 0.596110701560974
0.453515979186149 0.596404671669006
0.460732856107644 0.596713006496429
0.467949733029139 0.597035884857178
0.475166609950633 0.597373187541962
0.482383486872128 0.597724854946136
0.489600363793623 0.598091006278992
0.496817240715117 0.598471343517303
};
\addplot [line width=1.5pt, red]
table {%
0.204698407507712 0.59209563434124
0.204698407507712 0.598774948716164
};
\addplot [line width=1.5pt, color0, dashed]
table {%
0.2 0.59209563434124
0.2 0.598774948716164
};
\end{axis}

\end{tikzpicture}


==> figures/diffable_prior/diff_inferred_params_outputscale.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Output Scale},
xmin=-0.520911949125796, xmax=10.4343094087474,
xtick style={color=black},
xtick={-2,0,2,4,6,8,10,12},
y grid style={white!69.0196078431373!black},
ylabel={Cross Entropy Loss},
ymin=0.582872980833054, ymax=0.701910501718521,
ytick style={color=black},
ytick={0.6,0.64,0.68},
mystylepalette,
mystylepalettehptuning,
]
\addplot [line width=1.5pt, color0]
table {%
-0.0229473419497435 0.696499705314636
0.121390225347663 0.690717697143555
0.26572779264507 0.678760707378387
0.410065359942476 0.658001005649567
0.554402927239883 0.631062805652618
0.698740494537289 0.607101380825043
0.843078061834696 0.593039512634277
0.987415629132102 0.588283777236938
1.13175319642951 0.589252412319183
1.27609076372692 0.593126535415649
1.42042833102432 0.598241329193115
1.56476589832173 0.603675186634064
1.70910346561914 0.608952581882477
1.85344103291654 0.613865792751312
1.99777860021395 0.618356108665466
2.14211616751135 0.622434914112091
2.28645373480876 0.626136600971222
2.43079130210617 0.629497170448303
2.57512886940357 0.632546842098236
2.71946643670098 0.635312855243683
2.86380400399839 0.637821853160858
3.00814157129579 0.640102207660675
3.1524791385932 0.642183840274811
3.29681670589061 0.644097208976746
3.44115427318801 0.645871877670288
3.58549184048542 0.647534847259521
3.72982940778283 0.649109959602356
3.87416697508023 0.65061753988266
4.01850454237764 0.652073979377747
4.16284210967505 0.653492569923401
4.30717967697245 0.6548832654953
4.45151724426986 0.65625262260437
4.59585481156727 0.657604217529297
4.74019237886467 0.658938646316528
4.88452994616208 0.660254061222076
5.02886751345949 0.661546170711517
5.17320508075689 0.662808656692505
5.3175426480543 0.664034426212311
5.46188021535171 0.66521543264389
5.60621778264911 0.666343867778778
5.75055534994652 0.667412281036377
5.89489291724392 0.668414354324341
6.03923048454133 0.669345617294312
6.18356805183874 0.670202434062958
6.32790561913614 0.67098343372345
6.47224318643355 0.671688854694366
6.61658075373096 0.672319948673248
6.76091832102836 0.672879874706268
6.90525588832577 0.673372209072113
7.04959345562318 0.673801243305206
7.19393102292058 0.674172222614288
7.33826859021799 0.674489974975586
7.4826061575154 0.674759924411774
7.6269437248128 0.674987018108368
7.77128129211021 0.67517626285553
7.91561885940762 0.675332129001617
8.05995642670502 0.675458967685699
8.20429399400243 0.675560891628265
8.34863156129984 0.675641238689423
8.49296912859724 0.675703406333923
8.63730669589465 0.675750255584717
8.78164426319206 0.675784289836884
8.92598183048946 0.67580771446228
9.07031939778687 0.675822496414185
9.21465696508428 0.675830483436584
9.35899453238168 0.67583292722702
9.50333209967909 0.675831198692322
9.6476696669765 0.675826251506805
9.7920072342739 0.675818920135498
9.93634480157131 0.675810039043427
};
\addplot [line width=1.5pt, red]
table {%
1.00797701587642 0.582872980833054
1.00797701587642 0.701910501718521
};
\addplot [line width=1.5pt, color0, dashed]
table {%
1 0.582872980833054
1 0.701910501718521
};
\end{axis}

\end{tikzpicture}


==> figures/diffable_prior/diffable_train_valid.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={$\V_2$ CE Loss},
xmin=0.598681551543045, xmax=0.603698003157137,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={$\V_1$ CE Loss},
ymin=0.578715537458658, ymax=0.583200332552195,
ytick style={color=black},
y tick label style={
        /pgf/number format/.cd,
        precision=3,
        /tikz/.cd
    },
x tick label style={
        /pgf/number format/.cd,
        precision=3,
        /tikz/.cd
    },
mystylepalette,
mystylepalette2,
]
\addplot [semithick, color0, mystyle]
table {%
0.602757403132867 0.581092887818813
0.601998944215629 0.580408185124397
0.601418055441915 0.579917918145657
0.601015932934017 0.579618851691484
0.60078166976419 0.579494604319334
0.600686301154142 0.579510099738836
0.600680441956739 0.579609767347574
0.600704315061472 0.579728523641825
0.60070831742974 0.579813619405031
0.600667324107216 0.579839178472757
0.600580356787054 0.579804875552654
0.600461038513755 0.57972590893507
0.600328293495945 0.579623353332281
0.600200159133089 0.579517601728439
0.600090102425643 0.579424401372671
0.600005435776346 0.579353343397379
0.599946864367444 0.579307157695293
0.599909322108237 0.579282432347536
0.599884184571553 0.579271745830774
0.599861745855638 0.579266238510609
0.599834004607128 0.579258315712214
0.599796254225835 0.579243573993444
0.599747751250255 0.57922131434083
0.599690936125663 0.579193791300058
0.599630277451812 0.579165389537811
0.59957079878267 0.579140480607748
0.59951674086707 0.579121885150671
0.599470523889272 0.579111318588257
0.599432472405689 0.57910819798708
0.599400815915088 0.579109644442797
0.599372521460969 0.579111723154783
0.599344213854293 0.579110239446163
0.599313196517071 0.579102166444063
0.599278139292586 0.579086074531078
0.599239275505652 0.579062545448542
0.599197924099102 0.579033671915531
0.599156124707387 0.579002346992493
0.599115725568667 0.578971516042948
0.59907795196133 0.578943405002356
0.599042971561454 0.578919391781092
};
\addplot [semithick, color1, mystyle]
table {%
0.602134629893972 0.581849144697189
0.601534647639005 0.58137612208724
0.601097220060777 0.58108058899641
0.600817418106052 0.580950002223253
0.600678956592265 0.580956828296185
0.600644157325127 0.581052462756634
0.600657468053455 0.581172292977571
0.600664771789191 0.581257140040398
0.600634082847712 0.581274903565645
0.600559534352957 0.581223366856575
0.600452436514351 0.581119024306536
0.600330759029912 0.580985527187586
0.600211985789392 0.580845784693956
0.600109060313933 0.580717871785164
0.600028518397285 0.580612961351871
0.599970360267527 0.580535075962544
0.599928928995315 0.580481712520122
0.599895590079986 0.580446347594261
0.599861507323019 0.580421295762062
0.599820318726861 0.580400288403034
0.599769483339422 0.580380222201347
0.599710190060491 0.580361056476831
0.599646256210244 0.580344801098108
0.599582545839402 0.580333938002586
0.599523435935986 0.580330307036638
0.599471614753105 0.580333809554577
0.599427460331698 0.580341971665621
0.599389335444691 0.580350461602211
0.59935409446456 0.58035401776433
0.599318472098331 0.580347751826048
0.59927995902087 0.580328631103039
0.599237722287677 0.580296024829149
0.599192387671495 0.580251682251692
0.599145809644643 0.580199026167393
0.599100070226253 0.580142312049866
0.599056849484237 0.58008525967598
0.599016855641895 0.580030833780766
0.598979726129649 0.57998049095273
0.598944437138888 0.579934640079737
0.598909572070959 0.579892968684435
};
\addplot [semithick, color2, mystyle]
table {%
0.603344128334096 0.582693996280432
0.602506142945922 0.581882059127092
0.6018456729243 0.581268834024668
0.60136486354227 0.580853265821934
0.601059023480938 0.580628808885813
0.600909221499246 0.580573142766952
0.600877903667944 0.580643339455128
0.600911704557283 0.580779682695866
0.600954969812717 0.580920576155186
0.600966852766519 0.581021064966917
0.600929585114426 0.581061260402203
0.600845470036171 0.581042945384979
0.60072855727405 0.580980743020773
0.600597041373958 0.580894246399403
0.600468327652435 0.580802630782127
0.600355801799772 0.580721374154091
0.600267476687322 0.580660544037819
0.600205456343841 0.580624413043261
0.600166527630419 0.580611689388752
0.600143673430596 0.580616928040981
0.600127838361932 0.580632598996162
0.600110658121352 0.580651078671217
0.600085926717337 0.580666764229536
0.600050671900414 0.580676836520433
0.600005213133231 0.580681392848492
0.599952456180234 0.580682851523161
0.59989671888096 0.580684674978256
0.599842526588817 0.580690275132656
0.59979357680648 0.580701829940081
0.599751962500871 0.580719925612211
0.599717904034318 0.580743072628975
0.599689960897881 0.580768066346645
0.599665525502392 0.580790908932686
0.599641586596869 0.580807620584965
0.599615718941299 0.580815098881721
0.599586526692218 0.580811982452869
0.599553846507048 0.58079858854413
0.599518638408306 0.580776908099651
0.599482606222131 0.580749980062246
0.599447533032116 0.580721111893654
};
\addplot [semithick, color3,mystyle]
table {%
0.603469982629224 0.582996478229761
0.602650645778191 0.582198560535908
0.602005037688175 0.581591256707907
0.601534693672949 0.581173492223024
0.601233531359811 0.580937608629465
0.601082781899948 0.580862326025963
0.601045837245729 0.580907656848431
0.601070230674683 0.581017183959484
0.601100877193468 0.581131723672152
0.601097212230064 0.581207557320595
0.601042390059756 0.581225960403681
0.600939767245127 0.581189780384302
0.60080462561122 0.581114860475063
0.600656063542986 0.581021599620581
0.600511966805373 0.580929475426674
0.600385753247811 0.580853591710329
0.600284812401752 0.5808030590415
0.600210275729092 0.580780495852232
0.600157705230676 0.5807826846838
0.600118987528341 0.580802338570356
0.600084638793249 0.580830553621054
0.60004635611359 0.580859196037054
0.599998618495099 0.580882752686739
0.599939601647915 0.580899072140455
0.599870832028742 0.580909257233143
0.599796126007425 0.580916615277529
0.599720254084285 0.580925603061914
0.599647605145464 0.580940728485584
0.599580669053355 0.580964615643024
0.599518020390248 0.580992538183927
0.599457242241015 0.581008785516024
0.599403618435774 0.581009292751551
0.599360154257441 0.581017154604197
0.599318027724417 0.581041091531515
0.599273543120647 0.581058191210032
0.599225928322697 0.581067849546671
0.59917722345919 0.581072359979153
0.599128132838072 0.581073562651873
0.599080646562637 0.581074182540178
0.599036669016493 0.581076688170433
};
\end{axis}

\end{tikzpicture}


==> figures/overview_figures/diffhptuning.tex <==
\begin{tikzpicture}[
sample/.style={-stealth,decorate,decoration={snake}},
input/.style={-stealth},
]
	\node[] (valset) {$\mathbb{V}_1$};
	\node[] (data_sample) [right=of valset] {$D_{train} \cup \{x_{val},y_{val}\}$};
	\node[] (pfn) [above right=of data_sample, xshift=-2cm, yshift=-1cm,rectangle,align=left] {$q_{\theta}(y_{val}|x_{val},D_{train},\textcolor{orange}{\psi})$};
	\node[] (loss) [below=of pfn, yshift=.5cm] {CE$(\cdot,\cdot)$};
	
	\draw[sample] (valset.east) -- (data_sample.west) node[midway, below] {sample};
	\draw[input] ([xshift=-1cm]data_sample.north) |- ([yshift=0cm]pfn.west);
	\draw[input] ([xshift=.2cm]data_sample.north) |- ([yshift=-.1cm]pfn.west);
	\draw[input] ([xshift=1cm]data_sample.south) |- ([yshift=0cm]loss.west);
	\draw[input] (pfn.south) -- (loss.north);

	
\end{tikzpicture}

==> figures/overview_figures/training.tex <==
\begin{tikzpicture}[
sample/.style={-stealth,decorate,decoration={snake}},
input/.style={-stealth},
]
  \node[] (style_prior) {$p(\psi)$};
  \node[] (style) [right=of style_prior] {$\psi$};
  \node[] (prior) [below=of style,yshift=.7cm] {$p(D_{train} \cup \{x_{val},y_{val}\} | \psi)$};
  \node[] (data_sample) [right=of prior] {$D_{train} \cup \{x_{val},y_{val}\}$};
  \node[] (pfn) [above right=of data_sample, xshift=-2cm,yshift=-.8cm, rectangle,align=left] {$q_{\textcolor{orange}{\theta}}(y_{val}|x_{val},D_{train},\psi)$};
  \node[] (loss) [below=of pfn, yshift=.4cm] {CE$(\cdot,\cdot)$};
  
  \draw[sample] (style_prior.east) -- (style.west) node[midway, below] {sample};
  \draw[input] (style.south) -- (prior.north) node[midway, above] {};
  \draw[sample] (prior.east) -- (data_sample.west) node[midway, below] {sample};
  \draw[input] (style.east) -- ([yshift=.1cm]pfn.west) node[midway, above] {};
  \draw[input] ([xshift=-1cm]data_sample.north) |- ([yshift=0cm]pfn.west);
  \draw[input] ([xshift=.2cm]data_sample.north) |- ([yshift=-.1cm]pfn.west);
  \draw[input] ([xshift=1cm]data_sample.south) |- ([yshift=0cm]loss.west);
  
  \draw[input] (pfn.south) -- (loss.north);
  
\end{tikzpicture}

==> figures/overview_figures/transformer_visualization_only_train.tex <==
\iffalse
%\documentclass{article}
\usepackage[dvipsnames]{xcolor}
\usepackage{tikz}
\usetikzlibrary{positioning,calc,backgrounds,fit,arrows.meta}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.pathreplacing,calligraphy}


\fi
%\begin{document}
\newcommand{\lastidx}{n+1}
\newcommand{\evalidx}{n+1}
\newcommand{\setofpairs}[2]{\{(x_1^{#1}, y_1^{#1}),\dots,(x_{#2}^{#1}, y_{#2}^{#1})\}}
\newcommand{\seq}[1]{$\setofpairs{#1}{\lastidx{}}$}
\newcommand{\xypair}[1]{$(x_{#1},y_{#1})$}
\newcommand{\qattbend}{40}
\def\innerdistance{2.2em}
\def\outdistane{1.2em}
\def\indistane{1.em}
\begin{tikzpicture}[remember picture,
  inner/.style={circle,draw=blue!50,fill=blue!20,thick,inner sep=3pt},
]
\tikzstyle{bigbox} = [thick, fill=white, rounded corners, rectangle,draw=black!30]
\tikzstyle{sample} = [thick, minimum size=0.6cm, rounded corners,rectangle, fill=Salmon!10,draw=black!30]
\tikzstyle{loss} = [thick, minimum size=0.6cm, rounded corners,rectangle, fill=PineGreen!10,draw=black!30]
\tikzstyle{timestep} = [thick,minimum width=0.2cm,minimum height=.6cm, rounded corners,rectangle, fill=MidnightBlue!10,draw=black!30]
\tikzstyle{querytimestep} = [thick,minimum width=0.2cm,minimum height=.6cm, rounded corners,rectangle, fill=MidnightBlue!10,draw=black!30]
\tikzstyle{innerattention} = [draw=blue!30,-{Triangle[length=2mm, width=1mm]},]
\tikzstyle{queryattention} = [draw=red!30,-{Triangle[length=2mm, width=1mm]},]
\tikzstyle{output} = [draw=black!70,-{Triangle[length=2mm, width=1mm]},]
\tikzstyle{input} = [draw=black!70,-{Triangle[length=2mm, width=1mm]},]
\tikzstyle{every node} = [font=\footnotesize,]




\node[timestep] (t1) {};
\node[timestep, right=\innerdistance of t1] (t2) {};
\node[timestep, right=\innerdistance of t2] (t3) {};


\draw [ innerattention] (t1) to [bend left=15] (t2);
\draw [ innerattention] (t1) to [bend left=30] (t3);
\draw [ innerattention] (t2) to [bend right=15] (t1);
\draw [ innerattention] (t2) to [bend left=15] (t3);
\draw [ innerattention] (t3) to [bend right=30] (t1);
\draw [ innerattention] (t3) to [bend right=15] (t2);


\node[below=\indistane of t1] (i1) {\xypair{1}};
\draw [ input] (i1) -- (t1);
\node[below=\indistane of t2] (i2) {\xypair{2}};
\draw [ input] (i2) -- (t2);
\node[below=\indistane of t3] (i3) {\xypair{3}};
\draw [ input] (i3) -- (t3);

%\draw [pen colour={black!70},
%    decorate, 
%    decoration = {calligraphic brace, mirror,
%        raise=.7em,
%        amplitude=5pt}] (i1.west) --  (i3.east)
%    node[pos=0.5,below=1.2em,black]{$D$};

\end{tikzpicture}
%\end{document}

==> figures/prior_graphs/meta_bnn.tex <==
% \documentclass{article}
% \usepackage{pgfplots}
% \usepackage{tikz}
% \usetikzlibrary{shapes,decorations,arrows,calc,arrows.meta,fit,positioning}
% \begin{document}
\begin{tikzpicture}[-Latex,auto,node distance =0.2 cm and 0.3 cm,semithick,
    state/.style ={ellipse, draw, minimum width = .7 cm, minimum height = 0.7 cm},every node/.style={scale=0.3},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}]
    \node[state,fill=gray!40!white] (1) {$x^{(1)}$};
    \node[state,fill=gray!40!white] (2) [right =of 1] {$x^{(2)}$};
    
    \node[state] (3) [above left =of 1,yshift=0.2cm, xshift=1cm] {$H_1$};
    \node[state] (4) [above =of 1, xshift=1cm] {$H_2$};
    \node[state] (5) [above =of 2, xshift=1cm] {$H_3$};
    
    \node[state] (8) [above =of 3] {$H_1$};
    \node[state] (9) [above =of 4] {$H_2$};
    \node[state] (10) [above =of 5] {$H_3$};
    
    \node[state] (7) [above =of 9,fill=gray!40!white] {$y$};

    \path (1) edge (3);
    \path (1) edge (4);
    \path (1) edge (5);
    \path (2) edge (3);
    \path (2) edge (4);
    \path (2) edge (5);
    
    \path (3) edge (8);
    \path (4) edge (8);
    \path (5) edge (8);
    \path (3) edge (9);
    \path (4) edge (9);
    \path (5) edge (9);
    \path (3) edge (10);
    \path (4) edge (10);
    \path (5) edge (10);
    
    \path (8) edge (7);
    \path (9) edge (7);
    \path (10) edge (7);
\end{tikzpicture}
\begin{tikzpicture}[-Latex,auto,node distance =0.3 cm and 0.3 cm,semithick,
    state/.style ={ellipse, draw, minimum width = .7 cm, minimum height = 0.7 cm},every node/.style={scale=0.3},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}]
    \node[state,fill=gray!40!white] (1) {$x^{(1)}$};
    \node[state,fill=gray!40!white] (2) [right =of 1] {$x^{(2)}$};
    \node[state] (3) [above left =of 1,yshift=0.2cm] {$H_1$};
    \node[state] (4) [above =of 1] {$H_2$};
    \node[state] (5) [above =of 2] {$H_3$};
    \node[state] (6) [above right =of 2,yshift=0.2cm] {$H_4$};
    \node[state] (7) [above =of 4,xshift=0.8cm,fill=gray!40!white] {$y$};

    \path (1) edge (3);
    \path (1) edge (4);
    \path (1) edge (5);
    \path (1) edge(6);
    \path (2) edge (3);
    \path (2) edge (4);
    \path (2) edge (5);
    \path (2) edge (6);
    
    \path (3) edge (7);
    \path (4) edge (7);
    \path (5) edge (7);
    \path (6) edge (7);
\end{tikzpicture}
\begin{tikzpicture}[-Latex,auto,node distance =0.3 cm and 0.15 cm,semithick,
    state/.style ={ellipse, draw, minimum width = .7 cm, minimum height = 0.7 cm},every node/.style={scale=0.3},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}]
    \node[state,fill=gray!40!white] (1) {$x^{(1)}$};
    \node[state,fill=gray!40!white] (2) [right =of 1] {$x^{(2)}$};
    \node[state] (3) [above left =of 1,yshift=0.2cm] {$H_1$};
    \node[state] (4) [above =of 1] {$H_2$};
    \node[state] (5) [above =of 2] {$H_3$};
    \node[state] (8) [left =of 3] {$H_2$};
    \node[state] (6) [above right =of 2,yshift=0.2cm] {$H_4$};
    \node[state] (9) [right =of 6] {$H_3$};
    \node[state] (7) [above =of 4,xshift=0.8cm,fill=gray!40!white] {$y$};

    \path (1) edge (3);
    \path (1) edge (4);
    \path (1) edge (5);
    \path (1) edge(6);
    \path (1) edge (8);
    \path (1) edge (9);
    \path (2) edge (3);
    \path (2) edge (4);
    \path (2) edge (5);
    \path (2) edge (6);
    \path (2) edge (8);
    \path (2) edge (9);
    
    \path (3) edge (7);
    \path (4) edge (7);
    \path (5) edge (7);
    \path (6) edge (7);
    \path (8) edge (7);
    \path (9) edge (7);
\end{tikzpicture}
% \end{document}

==> figures/tabular_results/tabular_results_table_numerical.tex <==
\begin{tabular}{@{\hskip 0mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 0mm}}
\toprule
{} &        LightGBM &        CatBoost &         XGBoost &          ASKL2.0 &        AutoGluon &  TabPFN$_{n.e.}$ &                    TabPFN &        TabPFN + AutoGluon \\
\midrule
balance-scale                    &          0.9938 &          0.9245 &          0.9939 &            0.997 &           0.9919 &           0.9965 &           \textbf{0.9973} &                    0.9958 \\
mfeat-fourier                    &          0.9786 &          0.9816 &          0.9803 &           0.9826 &  \textbf{0.9843} &           0.9767 &                    0.9811 &                    0.9838 \\
mfeat-karhunen                   &          0.9979 &          0.9986 &          0.9983 &           0.9975 &  \textbf{0.9987} &           0.9939 &                    0.9978 &                    0.9985 \\
mfeat-morphological              &          0.9601 &          0.9629 &          0.9612 &           0.9671 &           0.9698 &           0.9657 &                    0.9669 &           \textbf{0.9722} \\
mfeat-zernike                    &          0.9716 &          0.9759 &          0.9735 &           0.9812 &  \textbf{0.9908} &           0.9812 &                    0.9823 &                    0.9901 \\
diabetes                         &          0.8247 &          0.8383 &          0.8378 &           0.8343 &           0.8391 &           0.8412 &                     0.841 &           \textbf{0.8427} \\
vehicle                          &          0.9232 &          0.9302 &          0.9282 &           0.9504 &           0.9416 &           0.9568 &           \textbf{0.9589} &                    0.9538 \\
analcatdata_authorship           &          0.9999 &          0.9999 &          0.9997 &       \textbf{1} &           0.9993 &       \textbf{1} &                \textbf{1} &                \textbf{1} \\
pc4                              &          0.9301 &          0.9413 &          0.9291 &           0.9331 &           0.9428 &           0.9298 &                    0.9383 &            \textbf{0.944} \\
pc3                              &          0.8178 &          0.8247 &          0.8288 &           0.8265 &           0.8282 &           0.8308 &           \textbf{0.8373} &                     0.836 \\
kc2                              &          0.8141 &          0.8323 &          0.8227 &           0.8311 &           0.8242 &           0.8322 &           \textbf{0.8346} &                    0.8321 \\
pc1                              &          0.8321 &            0.86 &          0.8489 &           0.8527 &           0.8578 &   \textbf{0.877} &                    0.8761 &                    0.8739 \\
banknote-authentication          &      \textbf{1} &      \textbf{1} &      \textbf{1} &       \textbf{1} &       \textbf{1} &       \textbf{1} &                \textbf{1} &                \textbf{1} \\
blood-transfusion-service-center &          0.7144 &          0.7403 &          0.7312 &           0.7504 &           0.7364 &            0.753 &           \textbf{0.7549} &                    0.7469 \\
qsar-biodeg                      &          0.9126 &          0.9217 &          0.9191 &           0.9247 &           0.9276 &  \textbf{0.9345} &                    0.9336 &                    0.9336 \\
wdbc                             &          0.9904 &          0.9931 &          0.9904 &           0.9947 &           0.9956 &            0.996 &           \textbf{0.9964} &                     0.996 \\
steel-plates-fault               &          0.9626 &          0.9655 &          0.9656 &  \textbf{0.9694} &           0.9666 &           0.9619 &                    0.9655 &                    0.9687 \\
climate-model-simulation-crashes &          0.9286 &          0.9344 &          0.9255 &           0.9291 &           0.9391 &  \textbf{0.9426} &                    0.9415 &                    0.9421 \\
\midrule
Wins AUC OVO
                                                     &               0 &               0 &               0 &                0 &                1 &                3 &                \textbf{4} &                         3 \\
Wins Acc.                        &               0 &               1 &               1 &                0 &                1 &                0 &                \textbf{6} &                         4 \\
Wins CE                          &               0 &               1 &               0 &                1 &                3 &                1 &                         3 &                \textbf{7} \\
\midrule
M. rank AUC OVO
                                                  &          6.9722 &          4.9444 &          6.1944 &           4.4722 &                4 &           3.8056 &                    2.9444 &           \textbf{2.6667} \\
Mean rank Acc.                   &          6.8889 &          4.9722 &          6.0556 &           5.1667 &           3.8889 &           3.8889 &                    2.8889 &             \textbf{2.25} \\
Mean rank CE                     &          5.7778 &          5.4444 &               6 &           6.4167 &           3.1111 &           4.1389 &                    3.0278 &           \textbf{2.0833} \\
\midrule
Mean AUC OVO
                                                     &   0.92$\pm$.013 &  0.924$\pm$.011 &   0.924$\pm$.01 &  0.929$\pm$.0096 &   0.93$\pm$.0091 &  0.932$\pm$.0088 &  \textbf{0.934}$\pm$.0086 &  \textbf{0.934}$\pm$.0084 \\
Mean Acc.                        &  0.862$\pm$.012 &  0.864$\pm$.011 &  0.866$\pm$.011 &    0.87$\pm$.014 &    0.881$\pm$.01 &  0.873$\pm$.0095 &           0.879$\pm$.0089 &  \textbf{0.886}$\pm$.0094 \\
Mean CE                          &   0.75$\pm$.039 &  0.747$\pm$.029 &   0.759$\pm$.04 &   0.813$\pm$.073 &   0.714$\pm$.014 &   0.727$\pm$.021 &            0.716$\pm$.019 &   \textbf{0.711}$\pm$.014 \\
\midrule
Mean time (s) 
                                    &            \multirow{2}{*}{3280} &            \multirow{2}{*}{3746} &            \multirow{2}{*}{3364} &            \multirow{2}{*}{3601} &                    \multirow{2}{*}{3077} &  \textbf{0.9478} (CPU) &          26.80 (CPU) &                      3152 (CPU) \\
(Tune + Train + Predict)                                                                        &             &             &             &             &                     &  \textbf{0.0204} (GPU) &          0.4832 (GPU) &                      3077 (GPU) \\
\bottomrule
\end{tabular}

==> figures/tabular_results/tabular_results_table_small.tex <==
\begin{tabular}{@{\hskip 0mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 1mm}
l@{\hskip 0mm}}
\toprule
{} &        LightGBM &        CatBoost &         XGBoost &         ASKL2.0 &               AutoGluon &  TabPFN$_{n.e.}$ &          TabPFN &        TabPFN + AutoGluon \\
\midrule
\midrule
Wins AUC OVO
                                         &               0 &               0 &               2 &               2 &                       2 &                4 &      \textbf{5} &                \textbf{5} \\
Wins Acc.            &               0 &               2 &               2 &               3 &                       3 &                0 &               6 &                \textbf{8} \\
Wins CE              &               0 &               1 &               3 &               1 &                       7 &                1 &               6 &                \textbf{9} \\
\midrule
M. rank AUC OVO
                                      &          6.6167 &          4.9667 &          5.4167 &            4.05 &                  3.7833 &             4.65 &             3.7 &           \textbf{2.8167} \\
Mean rank Acc.       &          6.5333 &          4.9833 &          5.1833 &          4.8667 &                  3.8167 &           4.5333 &          3.6167 &           \textbf{2.4667} \\
Mean rank CE         &          5.7333 &             5.6 &          5.4667 &             5.8 &                  2.8667 &           4.6167 &          3.5333 &           \textbf{2.3833} \\
\midrule
Win/T/L AUC
                             vs Tab.. &          5/4/21 &          9/4/17 &          6/5/19 &         10/6/14 &                 13/4/13 &           4/8/18 &           --/--/-- &                    15/7/8 \\
Win/T/L Acc vs Tab.. &          6/0/24 &          9/1/20 &         11/0/19 &         11/2/17 &                 12/0/18 &           6/3/21 &           --/--/-- &                    19/3/8 \\
Win/T/L CE vs TabP.. &          6/0/24 &          8/0/22 &          8/0/22 &          8/0/22 &                 20/0/10 &           1/4/25 &           --/--/-- &                    23/0/7 \\
\midrule
Mean AUC OVO
                                         &  0.884$\pm$.012 &   0.89$\pm$.011 &  0.891$\pm$.011 &   0.894$\pm$.01 &           0.895$\pm$.01 &    0.891$\pm$.01 &   0.894$\pm$.01 &  \textbf{0.898}$\pm$.0097 \\
Mean Acc.            &  0.815$\pm$.014 &  0.818$\pm$.011 &  0.821$\pm$.013 &  0.821$\pm$.016 &           0.83$\pm$.012 &    0.82$\pm$.013 &  0.825$\pm$.012 &   \textbf{0.834}$\pm$.011 \\
Mean CE              &  0.782$\pm$.074 &  0.767$\pm$.061 &  0.758$\pm$.047 &   0.815$\pm$.06 &  \textbf{0.72}$\pm$.015 &   0.742$\pm$.021 &  0.732$\pm$.018 &            0.721$\pm$.015 \\
\midrule
Mean time (s) 
                                    &            \multirow{2}{*}{3241} &            \multirow{2}{*}{3718} &            \multirow{2}{*}{3304} &            \multirow{2}{*}{3601} &                    \multirow{2}{*}{3127} &  \textbf{0.8688} (CPU) &          24.57 (CPU) &                      3152 (CPU) \\
(Tune + Train + Predict)                                                                        &             &             &             &             &                     &  \textbf{0.0187} (GPU) &          0.5335 (GPU) &                      3128 (GPU) \\
\bottomrule
\end{tabular}

==> figures/tabular_results/tabular_results_table_small_no_ens.tex <==
\begin{tabular}{llllllll}
\toprule
{} &           LogReg &         CatBoost &          XGBoost &          ASKL2.0 &                AutoGluon & TabPFN (No ens.) &           TabPFN \\
\midrule
balance-scale        &            0.962 &           0.9245 &           0.9939 &            0.997 &                   0.9919 &           0.9965 &  \textbf{0.9973} \\
mfeat-fourier        &           0.9763 &           0.9816 &           0.9803 &           0.9826 &          \textbf{0.9843} &           0.9767 &           0.9814 \\
breast-w             &           0.9938 &           0.9931 &           0.9896 &  \textbf{0.9939} &                   0.9933 &           0.9931 &           0.9934 \\
mfeat-karhunen       &           0.9954 &           0.9986 &           0.9983 &           0.9975 &          \textbf{0.9987} &           0.9939 &           0.9981 \\
mfeat-morphologica.. &           0.9637 &           0.9629 &           0.9612 &           0.9671 &          \textbf{0.9698} &           0.9657 &            0.967 \\
mfeat-zernike        &           0.9792 &           0.9759 &           0.9735 &           0.9812 &          \textbf{0.9908} &           0.9812 &           0.9823 \\
cmc                  &           0.6755 &           0.7256 &           0.7299 &  \textbf{0.7378} &                   0.7331 &           0.7233 &           0.7278 \\
credit-approval      &           0.9121 &           0.9389 &  \textbf{0.9422} &           0.9406 &                   0.9415 &           0.9253 &           0.9324 \\
credit-g             &            0.768 &           0.7852 &           0.7853 &            0.793 &          \textbf{0.7941} &           0.7894 &           0.7896 \\
diabetes             &           0.8373 &           0.8383 &           0.8378 &           0.8343 &                   0.8391 &  \textbf{0.8412} &            0.841 \\
tic-tac-toe          &           0.9945 &           0.9992 &       \textbf{1} &           0.9943 &               \textbf{1} &           0.9547 &           0.9758 \\
vehicle              &           0.9453 &           0.9302 &           0.9282 &           0.9504 &                   0.9416 &           0.9568 &  \textbf{0.9589} \\
eucalyptus           &           0.8852 &           0.8979 &           0.9004 &           0.9132 &                   0.9204 &           0.9218 &  \textbf{0.9245} \\
analcatdata_author.. &       \textbf{1} &           0.9999 &           0.9997 &       \textbf{1} &                   0.9993 &       \textbf{1} &       \textbf{1} \\
analcatdata_dmft     &           0.5657 &           0.5589 &           0.5743 &           0.5752 &                   0.5657 &           0.5643 &   \textbf{0.578} \\
pc4                  &           0.8909 &           0.9413 &           0.9291 &           0.9331 &          \textbf{0.9428} &           0.9298 &           0.9382 \\
pc3                  &            0.772 &           0.8247 &           0.8288 &           0.8265 &                   0.8282 &           0.8308 &   \textbf{0.837} \\
kc2                  &           0.8259 &           0.8323 &           0.8227 &           0.8311 &                   0.8242 &           0.8322 &  \textbf{0.8347} \\
pc1                  &           0.8209 &             0.86 &           0.8489 &           0.8527 &                   0.8578 &   \textbf{0.877} &           0.8763 \\
banknote-authentic.. &           0.9997 &       \textbf{1} &       \textbf{1} &       \textbf{1} &               \textbf{1} &       \textbf{1} &       \textbf{1} \\
blood-transfusion-.. &           0.7496 &           0.7403 &           0.7312 &           0.7504 &                   0.7364 &            0.753 &  \textbf{0.7549} \\
ilpd                 &           0.7088 &           0.7279 &           0.7171 &           0.7212 &                    0.723 &  \textbf{0.7412} &           0.7378 \\
qsar-biodeg          &           0.9202 &           0.9217 &           0.9191 &           0.9247 &                   0.9276 &  \textbf{0.9345} &           0.9338 \\
wdbc                 &           0.9946 &           0.9931 &           0.9904 &           0.9947 &                   0.9956 &            0.996 &  \textbf{0.9965} \\
cylinder-bands       &           0.8232 &           0.8757 &           0.8782 &           0.8718 &          \textbf{0.8878} &           0.8314 &           0.8337 \\
dresses-sales        &   \textbf{0.609} &           0.5696 &           0.5823 &           0.5705 &                   0.5507 &           0.5333 &           0.5376 \\
MiceProtein          &           0.9983 &           0.9999 &           0.9998 &           0.9999 &               \textbf{1} &           0.9997 &           0.9999 \\
car                  &           0.9827 &           0.9955 &           0.9948 &   \textbf{0.998} &                    0.997 &           0.9926 &           0.9947 \\
steel-plates-fault.. &            0.935 &           0.9655 &           0.9656 &  \textbf{0.9694} &                   0.9666 &           0.9619 &           0.9655 \\
climate-model-simu.. &           0.9317 &           0.9344 &           0.9255 &           0.9291 &                   0.9391 &  \textbf{0.9426} &           0.9417 \\
\midrule
Wins AUC OVO
                                         &                1 &                0 &                1 &                3 &               \textbf{6} &                4 &       \textbf{6} \\
Wins Acc.            &                2 &                1 &                2 &                4 &                        7 &                0 &       \textbf{9} \\
\midrule
Win/T/L AUC
                             vs Us    &           3/2/25 &           8/5/17 &           5/6/19 &          10/6/14 &                  13/4/13 &           4/7/19 &            0/0/0 \\
Win/T/L Acc vs Us    &           6/1/23 &           9/0/21 &          10/0/20 &          11/1/18 &                  11/1/18 &           5/4/21 &            0/0/0 \\
\midrule
Mean AUC OVO
                                         &  0.881$\pm$0.011 &   0.89$\pm$0.011 &  0.891$\pm$0.011 &   0.894$\pm$0.01 &  \textbf{0.895}$\pm$0.01 &   0.891$\pm$0.01 &   0.894$\pm$0.01 \\
Mean Acc.            &  0.809$\pm$0.013 &  0.818$\pm$0.011 &  0.821$\pm$0.013 &  0.821$\pm$0.016 &  \textbf{0.83}$\pm$0.012 &   0.82$\pm$0.013 &  0.826$\pm$0.012 \\
\midrule
M. rank AUC OVO
                                      &           5.5333 &             4.35 &              4.8 &           3.4167 &                   3.1333 &           3.8333 &  \textbf{2.9333} \\
Mean rank Acc.       &           5.1333 &           4.3167 &           4.6167 &             4.05 &                   3.2833 &             3.75 &    \textbf{2.85} \\
\midrule
Mean time (s) 
                                    &               60 &             3718 &             3304 &             3601 &                     3127 &  \textbf{0.0187} &             1.08 \\
\bottomrule
\end{tabular}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old_intro.tex <==
Many real-world applications in medicine, finance, research, predictive maintenance or sensor data modelling rely on strong Machine Learning (ML) algorithms for tabular data. 
%
While neural networks excel on many ML tasks, Gradient-Boosted Decision Trees (GBDT) still dominate the landscape of supervised ML for tabular data~\citep{GBDT,nnsfortabular2}, largely due to their short training time and robustness.

However, given that tree-based models are not differentiable, they cannot easily be composed and jointly trained with other blocks based on Deep Learning (DL).
% Furthermore, DL algorithms have been highly optimized to use efficient parallel computation devices such as GPUs and TPUs, potentially leading to large speedups over GBDT methods.
While many DL-based works claim superior performance for small and medium-sized datasets ($\approx$10\,000 samples), GBDT methods still outperform deep learning based approaches while also running significantly faster \citep{grinsztajn2022why}.

%In practical applications, h
Automated Machine Learning (AutoML) systems for tabular data have improved on GBDT approaches even 
%by yielding predictions at the push of a button
further~\citep{thornton-kdd13a,hutter-book19a,erickson-arxiv20a}. %  trading off human time with compute time in a specified time budget.% by automatically taking into account past performance on similar datasets, and by constructing ensembles from the models evaluated during the optimization.
% To achieve this, AutoML systems automatically evaluate and combine a large set of different ML algorithms, thus requiring substantial resources and becoming increasingly complex. % and take a long time to yield results.
State-of-the-art AutoML tools combine several classifiers (such as GBDTs and NNs), various preprocessing tools, advanced hyperparameter optimization methods~\citep{falkner-icml18a}, meta-learning~\citep{feurer-aaai15a,yang-kdd19a} and ensembling~\citep{escalante-jmlr09a,feurer-nips15a,olson-gecco16a,feurer-arxiv20v2,erickson-arxiv20a}. This, however, requires substantial resources, is not differentiable and becomes increasingly complex.
% These stacked complexities can lead to system failures on the user side~\citep{erickson-arxiv20a} that can be hard to understand.
%Thus, newer systems add even more complexity to catch these failures~\citep{feurer-arxiv20v2}.
%This complicated setup is run on the machine of the user.
AutoML systems are usually evaluated for several hours~\citep{gijsbers-automl2019,amlb}, and in our experiments, an AutoML training on a small dataset took at least a full minute, which makes real-time applications such as instant classification in a spreadsheet infeasible.

We propose a radical change, not only to tabular classifiers but the entire AutoML pipeline, that slashes the required time for training and hyperparameter tuning to \textit{a single second} and simplifies the application to a neural network (NN) forward-pass, a stable, differentiable and highly portable standard procedure. % that could even be run on handheld devices.
%that is highly portable and can be easily parallelized on compute architectures like GPUs.
%We do this by meta-learning a NN to become an AutoML system, which unlike previous work is probabilistically founded.

Our method builds on Prior-Data Fitted Networks (PFNs)~\citep{muller-iclr22a}, which learn the training and prediction algorithm itself.
PFNs approximate Bayesian inference given any prior one can sample from and yield the posterior predictive distribution (PPD) directly. 
% The PPD is a prediction distribution for unknown labels in our case, based on Bayesian reasoning.
Thus, PFNs approximate the probability distributions of classification labels by implicitly weighting all explanations for the data that are entailed in the prior.
%PFNs work for any prior that we are able to sample data from.
% By defining a Bayesian prior, the models inductive biases can be set explicitly.
While inductive biases in NNs and GBDTs depend on them being efficient to implement (e.g. through $L_2$ regularization, dropout \citep{srivastava14a} or limited tree-depth), in PFNs, one simply has to design a dataset generating algorithm encoding the desired prior. This fundamentally changes the way we can design learning algorithms.

In the original PFN paper~\citep{muller-iclr22a}, PPD approximation with PFNs was, amongst other experiments, demonstrated on binary classification for very small, balanced tabular datasets with only up to $30$ training examples and very few features.
We build on this work to create a state-of-the-art model for tabular multi-class classification tasks that we evaluate on real-world datasets with of up to $1\,000$ training samples, $100$ features and $10$ classes, comprising mixed feature types, missing data and unbalanced targets.

We use a prior based on Bayesian Neural Networks (BNNs; ~\citealt{neal-bayes96a,gal-phdthesis16a}) and Structural Causal Models (SCMs;~\citealt{pearl_2009,causalinferencelearningbook}) to model complex feature dependencies and potential causal mechanisms underlying tabular data.
Our prior also takes ideas from Occam\textquotesingle{s} razor: explanations based on simpler SCMs and BNNs have a higher likelihood in our prior.
In our prior, we define the hyperparameters describing our priors hypotheses via probability distributions, e.g. a Normal distribution for the average number of nodes in data-generating SCMs.
% We define our priors via probability distributions, e.g. a Normal distribution for the number of SCM nodes or a multinomial distribution for activation functions. To generate datasets for prior-fitting, we then sample from these distributions to obtain instantiations of concrete SCMs or BNNs (hypotheses) which we can use to generate data (see \ref{sec:prior_fitted_intro}).
% The resulting PPD implicitly models uncertainty over these hyperparameters, weighting them by their likelihood given the data and their prior probability.
The resulting PPD implicitly models uncertainty over these hyperparameters, weighting them by their likelihood given the data and their prior probability.
By obtaining the PPD, \methodname{} approximates an infinitely large ensemble of hyperparameters in a single forward-pass and requires no cross-validation.

Finally, we analyze the performance and behavior of the \methodname{} on different tasks and compare it to previous approaches for tabular classification on small datasets. We find that our method yields distinctly different predictions compared to existing approaches, likely due to the novelty and inductive biases introduced.
% By assuming a causal structure and a notion of simplicity in our prior, the PFN performs Bayesian inference over a space of hypotheses that is modelled through a structural causal framework and weighted by simplicity.

% Common regularization techniques to mitigate overfitting include data augmentation [1, 2], dropout [3, 4, 5], adversarial training [6], label smoothing [7], and layer-wise strategies [8, 9, 10] to name a few. However, these methods are agnostic of the causal relationships between variables limiting their potential to identify optimal predictors based on graphical topology, such as the causal parents of the target variable.

% Finally, since there are many decisions to be made when building a prior like this, we broadly hyperparameterize our prior, learn a single NN to support this broad prior and accept hyperparameters of the prior during inference time. We introduce a gradient-based methodology to tune these hyperparameters post hoc on real (meta-validation) datasets. 
% in a fully trained neural network.
%and even allow gradient-based methods to tune these hyperparameters. 
% This simplifies the development of PFN priors and reduces the number of models to be trained to one.
\iffalse
In this paper, we make the following contributions:
\begin{itemize}
    \item We present a state-of-the-art AutoML method for small, tabular datasets that yields more than $1000\times$ speedup over previous methods.
    \item We demonstrate the applicability of PFNs to real-world tasks. The PFN approach makes designing learning algorithms with explicit inductive biases possible by defining a prior sampling scheme.
    \item We introduce a prior over a large family of Structural Causal Models.
    \item We show that combining distinct priors is viable for PFNs and improves real-world performance.
    \item We show that the novelty and inductive biases of our approach lead to distinct predictions compared to baseline approaches, making it an ideal candidate for ensembling.
    \item We analyze the performance and behavior of the \methodname{} on different tasks and compare it to previous approaches for tabular classification.
\end{itemize}
\fi

% 30s per small dataset is usual in SOTA, we do 0.5s
% half a minute to half a second 

==> older_intro.tex <==
%%Many real-world applications in medicine, finance, research, predictive maintenance or sensor data modelling rely on strong Machine Learning (ML) algorithms for tabular data. 
%%
%%While neural networks excel on many ML tasks, Gradient-Boosted Decision Trees (GBDT) still dominate the landscape of supervised ML for tabular data~\citep{GBDT,nnsfortabular2}, largely due to their short training time and robustness.
%%
%%However, given that tree-based models are not differentiable, they cannot easily be composed and jointly trained with other blocks based on Deep Learning (DL).
% Furthermore, DL algorithms have been highly optimized to use efficient parallel computation devices such as GPUs and TPUs, potentially leading to large speedups over GBDT methods.
%While many DL-based works claim superior performance for small and medium-sized datasets ($\approx$10\,000 samples), GBDT methods still outperform deep learning based approaches while also running significantly faster \citep{grinsztajn2022why}.
%%
%%While many recent works try to fix this problem with a native DL approach for tabular classification~\citep{add_lots_of_citations}, we go one step further and simply apply a pre-trained DL model.
%%
%%
%%This is mainly due to competitive performance, short training times and robustness, however, the user is still left with many design decisions.
%
%% TODO somewhere in intro: How did we evaluate, Say that we did analysis on our method, include references to the corresponding sections.
%%
%%\todo{I would move this paragraph later; essentially, the real comparison is between TabPFN and a normal classification approach (which is then improved/combined in AutoML).}
%In practical applications, h
%%Automated Machine Learning (AutoML) systems for tabular data have improved on GBDT approaches even 
%by yielding predictions at the push of a button
%%further~\citep{thornton-kdd13a,hutter-book19a,erickson-arxiv20a}. %  trading off human time with compute time in a specified time budget.% by automatically taking into account past performance on similar datasets, and by constructing ensembles from the models evaluated during the optimization.
% To achieve this, AutoML systems automatically evaluate and combine a large set of different ML algorithms, thus requiring substantial resources and becoming increasingly complex. % and take a long time to yield results.
%%State-of-the-art AutoML tools combine several classifiers (such as GBDTs and NNs), various preprocessing tools, advanced hyperparameter optimization methods~\citep{falkner-icml18a}, meta-learning~\citep{feurer-aaai15a,yang-kdd19a} and ensembling~\citep{escalante-jmlr09a,feurer-nips15a,olson-gecco16a,feurer-arxiv20v2,erickson-arxiv20a}. This, however, requires substantial resources, is not differentiable and becomes increasingly complex.
% These stacked complexities can lead to system failures on the user side~\citep{erickson-arxiv20a} that can be hard to understand.
%Thus, newer systems add even more complexity to catch these failures~\citep{feurer-arxiv20v2}.
%This complicated setup is run on the machine of the user.
%%AutoML systems are usually evaluated for several hours~\citep{gijsbers-automl2019,amlb}, and in our experiments, an AutoML training on a small dataset took at least a full minute, which makes real-time applications such as instant classification in a spreadsheet infeasible.
%%
%%We propose a radical change to how tabular classification is usually done (namely fitting a new model from scratch to the training portion of a new dataset). We replace this step by performing a single forward pass on a large model that has been pre-trained to solve probabilistic classification tasks which are generated from a prior over what tabular datasets typically look like, integrating principles of simplicity and causal reasoning.
%%Next to slashing the time to solve tabular classification tasks to less than a second, this %%
%%but the entire AutoML pipeline, that slashes the required time for training and hyperparameter tuning to \textit{less than a second} and simplifies the application to a neural network (NN) forward-pass, a stable, differentiable and highly portable standard procedure.
%%
%%%We propose a radical change, not only to tabular classifiers but the entire AutoML pipeline, that slashes the required time for training and hyperparameter tuning to \textit{less than a second} and simplifies the application to a neural network (NN) forward-pass, a stable, differentiable and highly portable standard procedure. % that could even be run on handheld devices.
%that is highly portable and can be easily parallelized on compute architectures like GPUs.
%We do this by meta-learning a NN to become an AutoML system, which unlike previous work is probabilistically founded.
%%
%%Our method builds on Prior-Data Fitted Networks (PFNs)~\citep{muller-iclr22a}, which learn the training and prediction algorithm itself.
%%PFNs approximate Bayesian inference given any prior one can sample from and yield the posterior predictive distribution (PPD) directly. 
% The PPD is a prediction distribution for unknown labels in our case, based on Bayesian reasoning.
%%Thus, PFNs approximate the probability distributions of classification labels by implicitly weighting all explanations for the data that are entailed in the prior.
%PFNs work for any prior that we are able to sample data from.
% By defining a Bayesian prior, the models inductive biases can be set explicitly.
%%While inductive biases in NNs and GBDTs depend on them being efficient to implement (e.g. through $L_2$ regularization, dropout \citep{srivastava-jmlr14a} or limited tree-depth), in PFNs, one simply has to design a dataset generating algorithm encoding the desired prior. This fundamentally changes the way we can design learning algorithms.
%%
%%In the original PFN paper~\citep{muller-iclr22a}, PPD approximation with PFNs was, amongst other experiments, demonstrated on binary classification for very small, balanced tabular datasets with only up to $30$ training examples and very few features.
%%We build on this work to create a state-of-the-art model for tabular multi-class classification tasks that we evaluate on real-world datasets with of up to $1\,000$ training samples, $100$ features and $10$ classes, comprising mixed feature types, missing data and unbalanced targets.
%%
%%We use a prior based on Bayesian Neural Networks (BNNs; ~\citealt{neal-bayes96a,gal-phdthesis16a}) and Structural Causal Models (SCMs;~\citealt{pearl_2009,causalinferencelearningbook}) to model complex feature dependencies and potential causal mechanisms underlying tabular data.
%%Our prior also takes ideas from Occam\textquotesingle{s} razor: explanations based on simpler SCMs and BNNs have a higher likelihood in our prior.
%%In our prior, we define the hyperparameters describing our priors hypotheses via probability distributions, e.g. a Normal distribution for the average number of nodes in data-generating SCMs.
% We define our priors via probability distributions, e.g. a Normal distribution for the number of SCM nodes or a multinomial distribution for activation functions. To generate datasets for prior-fitting, we then sample from these distributions to obtain instantiations of concrete SCMs or BNNs (hypotheses) which we can use to generate data (see \ref{sec:prior_fitted_intro}).
% The resulting PPD implicitly models uncertainty over these hyperparameters, weighting them by their likelihood given the data and their prior probability.
%%The resulting PPD implicitly models uncertainty over these hyperparameters, weighting them by their likelihood given the data and their prior probability.
%%By obtaining the PPD, \methodname{} approximates an infinitely large ensemble of hyperparameters in a single forward-pass and requires no cross-validation.
%%
%%Finally, we analyze the performance and behavior of the \methodname{} on different tasks and compare it to previous approaches for tabular classification on small datasets. We find that our method yields distinctly different predictions compared to existing approaches, likely due to the novelty and inductive biases introduced.
% By assuming a causal structure and a notion of simplicity in our prior, the PFN performs Bayesian inference over a space of hypotheses that is modelled through a structural causal framework and weighted by simplicity.
%%
% Common regularization techniques to mitigate overfitting include data augmentation [1, 2], dropout [3, 4, 5], adversarial training [6], label smoothing [7], and layer-wise strategies [8, 9, 10] to name a few. However, these methods are agnostic of the causal relationships between variables limiting their potential to identify optimal predictors based on graphical topology, such as the causal parents of the target variable.
%%
% Finally, since there are many decisions to be made when building a prior like this, we broadly hyperparameterize our prior, learn a single NN to support this broad prior and accept hyperparameters of the prior during inference time. We introduce a gradient-based methodology to tune these hyperparameters post hoc on real (meta-validation) datasets. 
% in a fully trained neural network.
%and even allow gradient-based methods to tune these hyperparameters. 
% This simplifies the development of PFN priors and reduces the number of models to be trained to one.
%%
%%In this paper, we make the following contributions:
%%\begin{itemize}
    %%\item We present a state-of-the-art AutoML method for small, tabular datasets that yields more than $1000\times$ speedup over previous methods.
    %%\item We demonstrate the applicability of PFNs to real-world tasks. The PFN approach makes designing learning algorithms with explicit inductive biases possible by defining a prior sampling scheme.
    %%\item We introduce a prior over a large family of Structural Causal Models.
    %%\item We show that combining distinct priors is viable for PFNs and improves real-world performance.
    %%\item We show that the novelty and inductive biases of our approach lead to distinct predictions compared to baseline approaches, making it an ideal candidate for ensembling.
    %%\item We analyze the performance and behavior of the \methodname{} on different tasks and compare it to previous approaches for tabular classification.
%%\end{itemize}
